On the Role of Memory in Robust Opinion Dynamics

We investigate opinion dynamics in a fully-connected system, consisting of $n$ identical and anonymous agents, where one of the opinions (which is called correct) represents a piece of information to disseminate. In more detail, one source agent initially holds the correct opinion and remains with this opinion throughout the execution. The goal for non-source agents is to quickly agree on this correct opinion, and do that robustly, i.e., from any initial configuration. The system evolves in rounds. In each round, one agent chosen uniformly at random is activated: unless it is the source, the agent pulls the opinions of $\ell$ random agents and then updates its opinion according to some rule. We consider a restricted setting, in which agents have no memory and they only revise their opinions on the basis of those of the agents they currently sample. As restricted as it is, this setting encompasses very popular opinion dynamics, such as the voter model and best-of-$k$ majority rules. Qualitatively speaking, we show that lack of memory prevents efficient convergence. Specifically, we prove that no dynamics can achieve correct convergence in an expected number of steps that is sub-quadratic in $n$, even under a strong version of the model in which activated agents have complete access to the current configuration of the entire system, i.e., the case $\ell=n$. Conversely, we prove that the simple voter model (in which $\ell=1$) correctly solves the problem, while almost matching the aforementioned lower bound. These results suggest that, in contrast to symmetric consensus problems (that do not involve a notion of correct opinion), fast convergence on the correct opinion using stochastic opinion dynamics may indeed require the use of memory. This insight may reflect on natural information dissemination processes that rely on a few knowledgeable individuals.

==> trunks/Simulations.tex <==


\iffalse 
\subsection{Faster Dissemination with Memory} \label{sec:simulations}

In this section, we give experimental evidence suggesting that dynamics using a modest amount of memory can achieve consensus in an almost linear number of rounds.
When compared to memory-less dynamics, this represents an exponential gap (following the results of Section~\ref{sec:lower}).

\paragraph{``Follow the trend'': our candidate approach} The dynamics that we run in the simulations is derived from the algorithm of \cite{DBLP:conf/podc/KormanV22}, and uses a sample size of $\ell = 10 \, \log n$.
Each time an agent is activated, it decrements a countdown by 1. When the countdown reaches 0, the corresponding activation is said to be \textit{busy}.
On a busy activation,
the agent compares the number of opinions equal to 1 that it observes, to the number observed during the last busy activation.
\begin{itemize}
    \item If the current sample contains more 1's, then the agent adopts the opinion 1.
    \item Conversely, if it contains less 1's, then it adopts the opinion 0.
    \item If the current sample contains exactly as many 1's as the previous sample, the agent remains with the same opinion.
\end{itemize}
At the end of a busy activation, the agent resets its countdown to~$\ell$ (equal to the sample size) -- so that there is exactly one busy activation every $\ell$ activations. In addition, the agent memorizes the number of 1's that it observed, for the sake of performing the next busy activation. 

Overall, each agent needs to store two integers between $0$ and~$\ell$ (the countdown and the number of opinions equal to 1 observed during the last busy activation), so the dynamics requires $2\log(\ell) = \Theta(\log \log n)$ bits of memory.

The dynamics is described formally in Algorithm~\ref{algo:sequential_follow_the_trend}.

\begin{algorithm}[h!]
\SetKwInOut{Input}{Input}
\caption{Follow the Trend \label{algo:sequential_follow_the_trend}}
\DontPrintSemicolon
    {\bf Sample size:} $\ell = 10 \log n$ \;
    {\bf Memory:} $\cnt,\clk \in \{ 0,\ldots,\ell \}$ \;
    \Input{$k$, number of ones in a sample}% \\ $x_u$, opinion of $u$}
    \BlankLine

    \uIf{$\clk = 0$} {
        \;
        \uIf{$k < \cnt$}{
    		$x_u \leftarrow 0$ \;
    	}
    	\ElseIf{$k > \cnt$}{
    	    $x_u \leftarrow 1$ \;
         }\;
         $\cnt \leftarrow k$ \;
         $\clk \leftarrow \ell$ \;
    } \Else {
        $\clk \leftarrow \clk - 1$ \;
    }
\end{algorithm}

\paragraph{Experimental results}
Simulations were performed for~$n=2^i$, where $i \in \{3,\ldots,10\}$ for the Voter model, and $i \in \{3,\ldots,17\}$ for Algorithm~\ref{algo:sequential_follow_the_trend}, and repeated $100$ times each.
Every population contains a single source agent ($z=1$).
In self-stabilizing settings, it is not clear what are the worst initial configurations for a given dynamics. Here, we looked at two different ones:
\begin{itemize}
    \item a configuration in which all opinions (including the one of the source agent) are independently and uniformly distributed in~$\{0,1\}$,
    \item a configuration in which the source agent holds opinion~$0$, while all other agents hold opinion~$1$.
\end{itemize}

Results are summed up in Figure~\ref{fig:simulations_memory_short} in the main text, in terms of parallel rounds (one parallel round corresponds to~$n$ activations).
They are consistent with the theoretical insights of Section~\ref{sec:upper}.
Moreover, they suggest that the expected convergence time of our candidate dynamics is about~$\Theta(\polylog n)$ parallel rounds.

%\begin{figure}[htbp]
%    \centering
%    \includegraphics[width=0.6\textwidth]{resource/plot2.png}
%    \caption{\em
%    {\bf ``Follow the Trend'' versus the Voter model.}
%    Average convergence time (in parallel rounds) is depicted for different values of~$n$, over 100 iterations each, for $z=1$ source agent.
%    Blue lines with circular markers correspond to our candidate dynamics which is an adaptation of the ``follow the trend'' algorithm from \cite{DBLP:conf/podc/KormanV22}.
%    Orange lines with triangular markers correspond to the Voter Model.
%    Full lines depict initial configurations in which all opinions are drawn uniformly at random from~$\{0,1\}$.
%    Dotted lines depict initial configurations in which all opinions are taken to be different from the source agent.
%    }
%    \label{fig:simulations_memory}
%\end{figure}

\fi 

==> trunks/Upper_Bound.tex <==
\section{The Upper Bound} \label{sec:upper}

As defined in Section \ref{sec:prelim}, the Voter Model is the popular dynamics in which the   random node $v$, activated
at round $t$, pulls u.a.r. a random node $u \in V$ and updates his opinion to the opinion of $u$.

In this section, we prove that this dynamics converges within 
$\Theta(n^2 \log n)$ rounds in expectation. We prove the result for $z 
= 1$, noting that the upper bound can only improve for $z > 1$. 

\begin{theorem}\label{thm:uppbound}
If $z = 1$, the Voter Model achieves consensus to opinion $1$ within 
$2n^2H_{n-1} + \bigO(n^2)$ steps\footnote{$H_{\ell}$ denotes the 
$\ell$-th harmonic number.} in expectation and within $\bigO\left(n^2\log 
n\log\frac{1}{\delta}\right)$ steps with probability at least $1 - \delta$, 
for $0 < \delta < 1$. 
\end{theorem}
\begin{proof}
We first compute the general expression for $\Expec{z}{\hit_m}$, i.e., the 
expected time to reach state $n$ (thus, consensus) in $\mathcal{C}_2$ 
when the initial state is $z$, corresponding to the system starting in 
a state in which only the seed nodes hold opinion $1$. We then give a 
specific upper bound when $z = 1$. First of all, we 
note that, for $z$ seed nodes we have:
\[
	\Expec{z}{\hit_m} = \sum_{k = z + 1}^n\Expec{k-1}{\hit_k}.
\]
Considering the general expressions for the $\p_i$'s and 
$\q_i$'s for the birth-death chains we consider, we soon observe that for the Voter model,
\robin{$g_0 = g_1 =g$ (since the output does not depend on the opinion of the agent), with}
$\Expec{}{g(|S|)} = \frac{i}{n}$, whenever the 
number of nodes with opinion $1$ in the system is $i$. Hence for 
$\mathcal{C}_2$ we have:
\begin{align*}
	&\p_n = 0,\  \p_i = \frac{(n-i)i}{n^2}, \text{ for } i = 
	z,\ldots , n-1\\
	&\q_z = 0,\  \q_n = 1,\ \q_i = \frac{(n-i)(i-z)}{n^2}\text{, for } i = z + 1,\ldots , 
	n - 1
\end{align*}
The proof now proceeds along the following steps.

\paragraph{General expression for $\Expec{k-1}{\hit_k}$.}
For this first part, we proceed along the lines of \cite[Section 
2.5]{levin2017markov}. In a similar fashion, we define $w_0 = 1$ and, 
for $k = z + 1,\ldots , n$:
\[
	w_k = \prod_{i = z+1}^k\frac{\p_{i-1}}{\q_i}.
\]
Let $W = \sum_{j=z}^nw_j$ and $\pi_k = w_k/W$ for $k = z,\ldots , n$. 
Then $\{\pi_k\}_{k=z}^n$ is a probability distribution over the state 
space $\chi$ of $\mathcal{C}_2$. Moreover, proceeding like in \cite[Section 
2.5]{levin2017markov}, it is easy to see that the $w_k$'s (and thus, 
the $\pi_k$'s) satisfied the detailed balanced conditions for $k = 
z+1,\ldots, n$, namely:
\[
	\p_{k-1}w_{k-1} = \q_kw_k.
\]
To see this, note that, for $k\ge z+1$:
\[
	\p_{k-1}w_{k-1} = \p_{k-1}\prod_{i = 
	z+1}^{k-1}\frac{\p_{i-1}}{\q_i} = 
	\p_{k-1}\frac{\q_k}{\p_{k-1}}\prod_{i = z+1}^k\frac{\p_{i-1}}{\q_i} 
	= \q_kw_k.
\]
Hence, \cite[Proposition 1.20]{levin2017markov} implies that 
$\{\pi_k\}_{k=z}^n$ is also a stationary distribution for 
$\mathcal{C}_2$.

Proceeding like \cite[Section 2.5]{levin2017markov}, we then conclude 
that
\begin{equation}
	\Expec{k-1}{\hit_k} = \frac{1}{\q_kw_k}\sum_{j=z}^{k-1}w_j.
\end{equation}

\paragraph{Computing $\Expec{k-1}{\hit_k}$ for $\mathcal{C}_2$.}
First of all, considering the expressions of $\p_i$ and $\q_i$ for 
$\mathcal{C_2}$ we have, for $k = z + 1,\ldots , n - 1$:
\[
	w_k = \prod_{i=z+1}^{k}\frac{(n-i+1)(i-1)}{(i-z)(n-i)} = 
	\prod_{i=z+1}^{k}\frac{n-i+1}{n-i}\cdot\prod_{i=z+1}^{k}\frac{i-1}{i-z}.
\]
For the first term we have:
\[
	\prod_{i=z+1}^{k}\frac{n-i+1}{n-i} = \frac{n-z}{n-k},
\]
which follows by observing that this is a telescopic product in which 
all terms but the numerator of the first and the denominator of the 
last cancel out. As a result:
\[
	w_k = \frac{n-z}{n-k}f(k),
\]
where $f(k) = \prod_{i=z+1}^{k}\frac{i-1}{i-z}$. Finally, for $w_n$ we 
have:
\[
	w_n = w_{n-1}\frac{\p_{n-1}}{\q_n} = \frac{(n-z)(n-1)}{n^2}f(n-1),
\]
where the last equality follows since $\q_n = 1$ and by replacing the 
expression of $\p_{n-1}$ computer earlier.

\paragraph{The case $z = 1$.}
In this case, the formulas above simplify and we have, for $k = 
z+1,\ldots , n-1$:
\begin{align*}
	&\Expec{k-1}{\hit_k} = \frac{1}{\q_kw_k}\sum_{j=1}^{k-1}w_j = 
	\frac{n^2}{(k-1)f(k)}\sum_{j=1}^{k-1}\frac{f(j)}{n-j}\\
	& = \frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j},
\end{align*}
where the first equality follows by replacing $\q_k$ and $w_z,\ldots , 
w_k$ with their expressions for $\mathcal{C}_2$ computed above, while 
the second equality follows by observing that $f(z) = f(z+1) = \cdots = 
f(k) = 1$, whenever $z = 1$. Moreover, for $k = n$ we have:
\[
	\Expec{n-1}{\hit_n} = \frac{1}{\q_nw_n}\sum_{j=1}^{n-1}w_j = 
	\frac{n}{n-1}H_{n-1} = \bigO(\log n),
\]
where $H_{\ell}$ denotes the $\ell$-th harmonic number. In the 
derivation above, the first equality follows since for $z = 1$: i) $w_n 
= \left(\frac{n}{n-1}\right)^2$ and ii) we have:
\[
	\sum_{j=z}^{n-1}w_j = \sum_{j=1}^{n-1}\frac{n-1}{n-j} = 
	(n-1)H_{n-1}.
\]
We therefore have, for $z = 1$:
\begin{align*}
	&\Expec{1}{\hit_n} = \sum_{k=2}^n\Expec{k-1}{\hit_k} = 
	\sum_{k=2}^{n-1}\frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j} + 
	\bigO(\log n),
\end{align*}
where in the second equality we took into account that 
$\Expec{n-1}{\hit_n} = \bigO(\log n)$. We further write the first term 
of the right hand side as:
\begin{align*}
	&\sum_{k=2}^{n-1}\frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j}\\
	& = \sum_{k=2}^{\left\lfloor\frac{n}{2}\right\rfloor}\frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j} 
	+ \sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j}.
\end{align*}
When $k\le\left\lfloor\frac{n}{2}\right\rfloor$ we have $1/(n-j) <
2/n$ for every $j\le k - 1$, whence
\begin{align*}
	&\sum_{k=2}^{\left\lfloor\frac{n}{2}\right\rfloor}\frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j} < 
	\sum_{k=2}^{\left\lfloor\frac{n}{2}\right\rfloor}\frac{n^2}{k-1}\cdot\frac{2k}{n} = 
	2n\sum_{k=2}^{\left\lfloor\frac{n}{2}\right\rfloor}\frac{k}{k-1}\\
	& = 2n\sum_{k=2}^{\left\lfloor\frac{n}{2}\right\rfloor}\left(1 + 
	\frac{1}{k-1}\right) < n^2 + 2n\sum_{k=2}^{\left\lfloor\frac{n}{2}\right\rfloor} 
	\frac{1}{k-1}\\
	& = n^2 + 2nH_{\left\lfloor\frac{n}{2}\right\rfloor} = 
	n^2 + \bigO(n\log n).
\end{align*}
On the other hand, when $k\ge\left\lfloor\frac{n}{2}\right\rfloor + 1$ 
we have $\frac{n^2}{k-1}\le \frac{2n^2}{n-2}$, whence
\begin{align*}
	&\sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{n^2}{k-1}\sum_{j=1}^{k-1}\frac{1}{n-j}\le \sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{2n^2}{n-2}\sum_{j=1}^{k-1}\frac{1}{n-j}\\
	& = \sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{2n^2}{n-2}(H_{n-1} - H_{n-k}) < \sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{2n^2}{n-2}H_{n-1}\\
	& = \sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{2(n^2 - 4)}{n-2}H_{n-1} + \sum_{k=\left\lfloor\frac{n}{2}\right\rfloor + 
	1}^{n-1}\frac{8}{n-2}H_{n-1}\\
	& < 2n(n + 2)H_{n-1} + 4H_{n-1}.
\end{align*}
where the fourth equality and the fifth inequality follow from simple 
manipulations.
Overall, summing the contributions above, we have for $\Expec{1}{\hit_n}$ (and thus expected consensus time we 
have):
\[
	\Expec{1}{\hit_n} = 2n^2H_{n-1} + \bigO(n^2).
\]
To prove the second part of the claim, we use a standard argument. 
Consider $\lceil\ln\frac{1}{\delta}\rceil$ consecutive time intervals, 
each consisting of $s = \lceil\Expec{1}{\hit_n}\rceil = 2en^2H_{n-1} + \bigO(n^2)$ 
consecutive steps, with $e$ the base of natural logarithms. For $i = 1,\ldots , s - 1$, if the chain did not 
reach state $n$ in any of the first $i - 1$ intervals, then the 
probability that the chain does not reach state $n$ in the $i$ interval 
is at most $1/e$ by Markov's inequality. Hence, the probability that 
the chain does not reach state $n$ in any of the intervals is at most
\[
	\left(\frac{1}{e}\right)^{\ln\frac{1}{\delta}} = \delta.
\]
This concludes the proof.
\end{proof}

\paragraph{Remark.} It might seem reasonable to consider a different 
dynamics (generalizing the Voter Model), in which a node samples $k$ 
neighbours uniformly and independently at random and then it adopts 
opinion $1$ with probability $\ell/k$ if $\ell$ is the number of nodes 
with that opinion in the sample. It is easy to check that this change 
has no effect, in the sense that the transition probabilities of the 
corresponding birth-death chain do not change.  


